How stable are Transferability Metrics evaluations?

Transferability metrics is a maturing field with increasing interest, which aims at providing heuristics for selecting the most suitable source models to transfer to a given target dataset, without fine-tuning them all. However, existing works rely on custom experimental setups which differ across papers, leading to inconsistent conclusions about which transferability metrics work best. In this paper we conduct a large-scale study by systematically constructing a broad range of 715k experimental setup variations. We discover that even small variations to an experimental setup lead to different conclusions about the superiority of a transferability metric over another. Then we propose better evaluations by aggregating across many experiments, enabling to reach more stable conclusions. As a result, we reveal the superiority of LogME at selecting good source datasets to transfer from in a semantic segmentation scenario, NLEEP at selecting good source architectures in an image classification scenario, and GBC at determining which target task benefits most from a given source model. Yet, no single transferability metric works best in all scenarios.

==> 5_figures.tex <==

\begin{table}
    \centering
    \tiny
    {
        \begin{tabular}{l*{4}{c@{\hspace{0.7mm}}}}\toprule
        Dataset                      & Domain  & \# classes  & \# train & \# train \\
        & & & source  & target  \\
        \midrule
        Pascal Context~\cite{mottaghi14cvpr}  & Consumer              & 60        & 5K & 150 \\
        Pascal VOC~\cite{pascal-voc-2012} & Consumer              & 22   &  10K  & 150 \\
        ADE20K~\cite{zhou17cvpr}      & Consumer              & 150   &   20K & 1000\\
        COCO~\cite{caesar18cvpr,lin14eccv,kirillov19cvpr}       & Consumer  & 134 & 118K & 1000 \\
        KITTI~\cite{alhaija18ijcv}   & Driving & 30 & 150  & 150 \\
        CamVid~\cite{brostow09prl}    & Driving  & 23 & 367  & 150 \\
        CityScapes~\cite{cordts16cvpr}    & Driving  & 33   & 3K  & 150 \\
        IDD~\cite{varma19wacv} & Driving & 35 & 7K  & 150 \\
        BDD~\cite{yu20cvpr} & Driving & 20 & 7K  & 150 \\
        MVD~\cite{neuhold17cvpr} & Driving & 66 & 18K  & 150 \\
        ISPRS~\cite{rottensteiner14isprs}  & Aerial & 6 & 4K  & 150 \\
        iSAID~\cite{waqas2019isaid,xia18cvpr} & Aerial     & 16 & 27K  & 150 \\
        SUN RGB-D~\cite{song15cvpr} & Indoor & 37 & 5K  & 150 \\
        ScanNet~\cite{dai17cvpr} & Indoor & 41 & 19K  & 150 \\
        SUIM~\cite{islam2020suim} & Underwater & 8 & 1525  & 150 \\
        vKITTI2~\cite{cabon20arxiv,gaidon16cvpr} & Synthetic driving & 9 & 43K  & 150 \\
        vGallery~\cite{weinzaepfel19cvpr} & Synthetic indoor & 8 & 44K  & 150 \\
        \bottomrule
        \end{tabular}
    }
    \caption{Overview of the semantic segmentation datasets used for our transferability experiments. Including the domain, the number of classes and the number of training images when used as source or as target dataset in our low-shot transfer learning setting.}
    \label{tab:datasets}
\end{table}



==> table_target_selection_fixed.tex <==
\begin{table}[t]
\centering
\begin{tabular}{c|cccccc}
\hline
                  & \textbf{GBC} & \textbf{LEEP} & \textbf{NLEEP} & \textbf{LogMe} & \textbf{H-Score} & \textbf{NumClasses} \\
\textbf{Cifar100} & 0.580       & 0.304         & 0.470          & \textbf{0.675}        & 0.386            &   - \\
\textbf{Dogs} & \textbf{0.740}        & 0.703         & 0.611          & 0.521         & 0.191           &   -  \\
\textbf{Sun397} & 0.509        & 0.421         & \textbf{0.681}          & 0.263         & 0.256            &   - \\
\textbf{Flowers} & 0.344        & 0.266         & 0.341       & \textbf{0.388}         & 0.167           &   -\\ \hline
\textbf{Average} & \textbf{0.543}        & 0.424        & 0.526         & 0.462         & 0.250          &   -\\ \hline
\end{tabular}
\caption{Table X. \tm{Can we use the same datasets as in Figure 1?} \tm{Can we do sub-sample analysis?} \tm{The naming of the datasets should be consistent across tables and figures}
}
\label{tab:target_selection_fixed}
\end{table}

==> table_target_selection_random.tex <==
\begin{table}[t]
\centering
\begin{tabular}{c|cccccc}
\hline
                  & \textbf{GBC} & \textbf{LEEP} & \textbf{NLEEP} & \textbf{LogMe} & \textbf{H-Score} & \textbf{NumClasses} \\
\textbf{Cifar100} & \textbf{0.935}        & 0.909         & 0.933          & -0.787        & 0.686            &   0.899 \\
\textbf{Dogs} & 0.948        & \textbf{0.949}         & 0.936          & -0.789         & 0.200            &   0.913  \\
\textbf{Sun397} & \textbf{0.960}        & 0.947        & 0.950          & -0.920         & 0.473            &   0.953 \\
\textbf{Flowers} & \textbf{0.748}        & 0.699         & 0.712         & -0.628         & -0.642           &   0.697\\ \hline
\textbf{Average} &  \textbf{0.898}        & 0.876         & 0.883        & -0.781         & 0.179           &   0.866\\ \hline
\end{tabular}
\caption{Table X. \tm{Can we use the same datasets as in Figure 1?} \tm{Can we do sub-sample analysis?} \tm{The naming of the datasets should be consistent across tables and figures}
\tm{Probably put next to Table 8.}
\tm{Add at least one of those scatter plots, like Fig 4 from GBC paper.}
}
\label{tab:target_selection_random}
\end{table}
